Performance Analysis of Underlay Cognitive Radio Systems: Estimation-Throughput Tradeoff

In this letter, we study the performance of cognitive Underlay Systems (USs) that employ power control mechanism at the Secondary Transmitter (ST). Existing baseline models considered for the performance analysis either assume the knowledge of involved channels at the ST or retrieve this information by means of a feedback channel, however, such situations hardly exist in practice. Motivated by this fact, we propose a novel approach that incorporates the estimation of the involved channels at the ST, in order to characterize the performance of USs under realistic scenarios. Moreover, we apply an outage constraint that captures the impact of imperfect channel knowledge, particularly on the interference power received at the primary receiver. Besides this, we employ a transmit power constraint at the ST to determine an operating regime for the US. Finally, we analyze an interesting tradeoff between the estimation time and the secondary throughput allowing an optimized performance of the US.

==> figures/fig_opc_vs_SNR_diff_N_diff_maxContPow_th.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_opc_vs_SNR_diff_N_diff_maxContPow_th}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           31-Aug-2015 11:33:29
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\opc$\end{tabular}}%
\psfrag{s06}[t][t]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma$ [dB]\end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\tau = 10$ ms}%
\psfrag{s13}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\tau = 1$ ms}%
\psfrag{s14}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\tau = 10$ ms}%
%
% axes font properties:
\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-30}%
\psfrag{x02}[t][t]{-25}%
\psfrag{x03}[t][t]{-20}%
\psfrag{x04}[t][t]{-15}%
\psfrag{x05}[t][t]{-10}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
\psfrag{v10}[r][r]{0.9}%
\psfrag{v11}[r][r]{1}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_opc_vs_SNR_diff_N_diff_maxContPow_th.eps}}%
%\end{psfrags}%
%
% End fig_opc_vs_SNR_diff_N_diff_maxContPow_th.tex


==> figures/fig_opt_est_time_vs_SNR_AWGN.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_opt_est_time_vs_SNR_AWGN}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           24-Aug-2015 15:04:08
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s03}[b][b]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\ttau$ [ms]\end{tabular}}%
\psfrag{s04}[t][t]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma$ [dB]\end{tabular}}%
%
% axes font properties:
\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-15}%
\psfrag{x02}[t][t]{-10}%
\psfrag{x03}[t][t]{-5}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{5}%
\psfrag{x06}[t][t]{10}%
%
% yticklabels:
\psfrag{v01}[r][r]{1.5}%
\psfrag{v02}[r][r]{2}%
\psfrag{v03}[r][r]{2.5}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{3.5}%
\psfrag{v06}[r][r]{4}%
\psfrag{v07}[r][r]{4.5}%
\psfrag{v08}[r][r]{5}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_opt_est_time_vs_SNR_AWGN.eps}}%
%\end{psfrags}%
%
% End fig_opt_est_time_vs_SNR_AWGN.tex


==> figures/fig_opt_est_time_vs_SNR_fading.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_opt_est_time_vs_SNR_fading}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           19-Aug-2015 14:07:04
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s03}[b][b]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\ttau$ [ms]\end{tabular}}%
\psfrag{s04}[t][t]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma$ [dB]\end{tabular}}%
%
% axes font properties:
\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-15}%
\psfrag{x02}[t][t]{-10}%
\psfrag{x03}[t][t]{-5}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{5}%
\psfrag{x06}[t][t]{10}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_opt_est_time_vs_SNR_fading.eps}}%
%\end{psfrags}%
%
% End fig_opt_est_time_vs_SNR_fading.tex


==> figures/fig_opt_thr_vs_SNR_fading.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_opt_thr_vs_SNR_fading}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           19-Aug-2015 14:07:03
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s06}[b][b]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\rs(\ttau)$ [bits/sec/Hz]\end{tabular}}%
\psfrag{s07}[t][t]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma$ [dB]\end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Lemma 2}%
\psfrag{s14}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}IM}%
\psfrag{s15}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}EM}%
\psfrag{s16}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Lemma 2}%
\psfrag{s17}[b][b]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\rs(\ttau)$\end{tabular}}%
\psfrag{s18}[t][t]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma$\end{tabular}}%
\psfrag{s19}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Zoom\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.5}%
\psfrag{x03}[t][t]{1}%
\psfrag{x04}[t][t]{-15}%
\psfrag{x05}[t][t]{-10}%
\psfrag{x06}[t][t]{-5}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{5}%
\psfrag{x09}[t][t]{10}%
%
% yticklabels:
\psfrag{v01}[r][r]{1.8}%
\psfrag{v02}[r][r]{1.9}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{0}%
\psfrag{v05}[r][r]{1}%
\psfrag{v06}[r][r]{2}%
\psfrag{v07}[r][r]{3}%
\psfrag{v08}[r][r]{4}%
\psfrag{v09}[r][r]{5}%
\psfrag{v10}[r][r]{6}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_opt_thr_vs_SNR_fading.eps}}%
%\end{psfrags}%
%
% End fig_opt_thr_vs_SNR_fading.tex


==> figures/fig_thr_est_time_tradeoff_fading.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_thr_est_time_tradeoff_fading}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           21-Aug-2015 15:47:47
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\rs(\tau)$ [bits/sec/Hz]\end{tabular}}%
\psfrag{s06}[t][t]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\tau$ [ms]\end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Simulated}%
\psfrag{s13}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}IM}%
\psfrag{s14}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}EM}%
\psfrag{s15}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Lemma 2}%
\psfrag{s16}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\trs(\ttau)$}%
\psfrag{s17}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Simulated}%
%
% axes font properties:
\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{$10^{-3}$}%
\psfrag{x02}[t][t]{$10^{-2}$}%
\psfrag{x03}[t][t]{$10^{-1}$}%
\psfrag{x04}[t][t]{$10^{0}$}%
\psfrag{x05}[t][t]{$10^{1}$}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.8}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{1.2}%
\psfrag{v04}[r][r]{1.4}%
\psfrag{v05}[r][r]{1.6}%
\psfrag{v06}[r][r]{1.8}%
\psfrag{v07}[r][r]{2}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_thr_est_time_tradeoff_fading.eps}}%
%\end{psfrags}%
%
% End fig_thr_est_time_tradeoff_fading.tex

